Rubik: A Hierarchical Architecture for Efficient Graph Learning

Graph convolutional network (GCN) emerges as a promising direction to learn the inductive representation in graph data commonly used in widespread applications, such as E-commerce, social networks, and knowledge graphs. However, learning from graphs is non-trivial because of its mixed computation model involving both graph analytics and neural network computing. To this end, we decompose the GCN learning into two hierarchical paradigms: graph-level and node-level computing. Such a hierarchical paradigm facilitates the software and hardware accelerations for GCN learning. We propose a lightweight graph reordering methodology, incorporated with a GCN accelerator architecture that equips a customized cache design to fully utilize the graph-level data reuse. We also propose a mapping methodology aware of data reuse and task-level parallelism to handle various graphs inputs effectively. Results show that Rubik accelerator design improves energy efficiency by 26.3x to 1375.2x than GPU platforms across different datasets and GCN models.

==> tex/algorithm.tex <==
% \todo{a figure to show the whole design picture}
% \begin{figure*}[h]
%     \centering
%     \includegraphics[width=0.9\columnwidth]{fig/overview.pdf}
%     \caption{Design Overview.}
%     \label{fig: Graph Optimization Workflow.}
% \end{figure*}
\section{Graph Reordering}
In this section, we introduce the graph reordering methodology which improves the temporal reuse distance of the non-Euclidean data. With the reordered graph, we propose the mapping strategy considering both the data reuse optimization and task-level parallelism

\subsection{Overview}
As a major step of GNN computation, neighbor aggregation occupy \abanti{occupies a} large proportion of the overall running time. To improve its efficiency, a novel PE workload mapping generation (WMG) has been proposed to improve the accelerator on-chip cache hit rate while minimizing off-chip memory access overhead. As shown in Figure~\ref{fig: Workload Mapping Generation Workflow.}, our WMG workflow involves several key stages. First, for super (\abanti{I think 'super' is not very formal, use 'extremely'}) large graphs, we reduce their size through graph partitioning, which facilitates their transformation and mapping generation and keeping \abanti{helps keep} the information of their original graph structure.
\abanti{I have a consistent concern about an issue in this work. It is mentioned that super large graphs are tackled by partitioning. In reality, the graphs used in this work are not at all super large. The largest graph is only 114M edges, which is actually very small. First, I am concerned about the claim of 1) "super/extremely large" graphs. Second, I am concerned about the following: if 114M edges is "extremely large" for this accelerator, I wonder how scalable this accelerator is. Can Geom handle real-world billion-edge-scale graphs? I think this point should be discussed somewhere in the paper} Second, \abanti{the} graph transformation and optimization process reorganize \abanti{reorganizes the} adjacent \abanti{it is not 'adjacent' but 'adjacency'} matrix of subgraphs to increase computation reuse in aggregation. Third, workload output stage generates the workload mapping based on transformed subgraphs and distributes workloads to PEs in different schemes (e.g., sequential, node balance) \abanti{Please change 'adjacent' to 'adjacency' in Fig. 8. Also, in Fig. 8 do you mean "Meties" or "METIS"?}.

% improve the efficiency of GNN computation and memory access. Specifically, computation reuse GNN reduce the times of aggregation from neighborhood vertices information through caching the vertex-level partial sum, i.e., neighbors information shared by several nearby vertices can be aggregated only once and used multiple times before being expelled from the on-chip cache, as shown in Figure~\ref{}, vertex 2 and 3 share the same set of neighbors (vertex 1,4,5,6), therefore, during the aggregation step of GNN, the partial aggregation result of vertex 1,4,5,6 can be reused by 2,3 without re-computing. 
% On the other side, Data reuse improves the usage of the vertex information that are cached at on-chip buffer. Graph information are generally processed in the format of the adjacent matrix, for GNN aggregation the target vertex information can be aggregated towards the source vertex. Thus, if the consecutive rows (id-nearby vertex) share the same subset of the target neighbors, the memory access of those neighbors can be efficiently reduced. As shown in Figure~\ref{}, the vertex 4 and 5 share the same subset of vertex 5,6, and 7, since vertex 4 and 5 are processed consecutively, the information of vertex 5,6, and 7 only needs to be accessed once.

\subsection{Graph Partition}
In most real-world settings, graphs are large in size with huge \abanti{Once again, it is probably not OK to call the evaluation graphs in this paper (largest 114M edges) "huge"} number of vertices and edges, which is challenging to conduct graph data learning. Many GNN algorithms leverage the graph partition to cluster the nodes in subgraphs for better training efficiency~\cite{clusterGCN,chordalGNN}. To this end, WMG handles large graphs at the first step of its workflow, where a highly-efficient tool -- Meties~\cite{karypis1998fast}, is leveraged to partition the original graph into a set of subgraphs before the further processing \abanti{There are several well-known graph partitioning schemes. We need to justify why we choose METIS. Is there something about this accelerator which makes METIS a good fit?}. 

\subsection{Graph Reordering}

Graph reordering techniques exploit the structural properties to reassign index ID to vertex \abanti{vertices}, so that the layout changes to improve the locality of graph data~\cite{graphOrdering_IISWC18}. In our work, we propose a lightweight graph reordering techniques \abanti{technique} based on locality-sensitive hashing to determine the execution order and mapping location. The goal of reordering in our work is to group the nodes with more shared neighbors together to improve the temporal reuse when conducting the aggregation reduction.
The intrinsic reason that reordering method can provide better temporal reuse is based on the fact that real-world graphs exhibit a "community structure" ~\cite{Graphcommunity}, which means that some nodes share the neigbhors or have closer relationship than others. Therefore, by grouping them together, the data locality during execution will be significantly improved. To note, graph reordering does not change the graph structure but only affects the execution order of the graph. 

We develop the graph reordering algorithm by row-column transformation of the graph adjacency matrix. We incorporate \textit{Locality-Sensitivity Hashing} (LSH) and \textit{Row-Column Reordering} for graph reordering %and \textit{Run-length Encoding} (RLE) 
and adopt Run-length Encoding (RLE) length to quantify the effectiveness of ordered graphs.  


\noindent\textbf{Locality-sensitive Hashing.}
Locality-sensitive hashing (LSH)  is an algorithmic technique, being widely used to solve the approximate or exact nearest neighbor problem in high dimension space~\cite{LSH1,LSH2,LSH3}, that groups similar items into the same "buckets" with high probability. The basic concept based on random projection: for every input vector x, the hashing \abanti{hash} function is calculated by project \abanti{projecting} this vector x to several random vectors. With a series of random vectors, LSH maps an input vector to a bit vector (buckets). Input vectors with smaller distance have a higher probability to result in the same cluster with the same bit vector.  

\noindent\textbf{Row/Column Reordering.}
\abanti{I think readers could be confused here. I think LSH and row-column reordering are intertwined or SYNERGISTIC. They work TOGETHER to create a reordered graph. So, I believe there is no need to make separate headings for each. We created a heading called "Row-column ordering" but under this heading, we are still talking a lot about LSH. Instead it is better to make one heading "Synergistic Locality-sensitive Hashing and Row-Column Ordering" or "LSH at row and column levels of an adjacency matrix" and write the entire description under this one heading.}
We leverage LSH to cluster the nodes with more shared neighbors. Every row in the adjacency matrix of the graph is a vector that represents the neighbor connections for this vertex. Taking these vectors of rows in the adjacency matrix, LSH hashing groups the rows into several groups. Taking the detailed example in Figure~\ref{fig: Row-Column Reordering.} for illustration, Row-02 and Row-04 are grouped in cluster because they share most of the neighbors. Similarly, Row-05 and Row-08 are grouped in a cluster. Row-03, Row-01, Row-07, and Row-08 are grouped in a cluster. Thus, after the row transformation in step 1, we have the transformed graph with the nodes that assigned to the same buckets being placed continuously. Then we conduct the LSH clustering to the every column in this transformed adjacency matrix (step 2 in Figure~\ref{fig: Row-Column Reordering.}). We set a iteration limit so that this process can be iterated executed for better reordering effectiveness. 
%The column process is similar like that in the row transformation.   
%Specifically, the overall reordering process is illustrated as shown in Figure~\ref{fig: Row-Column Reordering.} with a detailed example, 
%where one iteration of row and column reordering on a graph adjacent matrix. The left-top adjacent matrix presents a graph connection among $node$ $01-05$. We  apply row reordering and column reordering in a interleave manner to minimize its column- and row-wise RLE respectively.

%Our mapping algorithm extends the use of LSH to explore the node neighborhood similarity that can maximize the data reuse in GNNs. As shown in Figure~\ref{fig: Row-Column Reordering.}, N-01, N-03, and N-05 aggregate from highly overlapped neighbor sets, thus, LSH assigns these three nodes into the same buckets. 

%And in the following row-column reordering stage, the nodes that assigned to the same buckets will be placed continuously for generating efficient workload mapping.
% algorithm process these two nodes consecutively which can maximize the computation reuse while increasing the cache hit rate. In order to organize the adjacent matrix in a way that can maximize the performance of the distance computation reuse, while minimizing overhead. 



\begin{comment}
\subsubsection{Reordering Algorithm}
Graph reordering algorithm of conducting Row/Column transformation is described in the Algorithm~\ref{alg: LSH-based Row/Column Reordering}. The input of the algorithm is a graph adjacent matrix (\textit{adjMat}), the signature length of LSH function (\textit{sigLen}), the size of node clusters (\textit{cluSize}), and the number of iteration (\textit{iterNo}), and the output is a transformed \textit{adjMat} with its corresponding row and column node ID order. 
\end{comment}

%The main iteration starts from \textit{line 6}, where we check the status of row/column change (\textit{rowColChange}) from last iteration and the iteration counter (\textit{iterNo}) for transformation control. 
%As shown in the Algorithm~\ref{alg: RLE encoding.}, the run-length encoding algorithm takes the input of adjacent matrix and axis sign to measure the row/column-wise density of adjacent matrix. The \textit{applyRLE} function return a list of RLE values for each row/column based on \textit{axisSign}(either 'row' or 'column'). While the \textit{Accumulate} function totals up the values in RLEList to get the overall row/column RLE of the input matrix. The RLE part takes the complexity of $O(S)$, where $S$ is total number of elements of an adjacent matrix.  
%As shown in the Algorithm~\ref{alg: LSH-based Row/Column Reordering}, the input of our graph reordering subroutine includes graph adjacent matrix, length of the hash signature, cluster size and axis sign (either 'row' or 'column'). The output is row-column reordered graph adjacent matrix, and its row and column order of node ids. 
\begin{comment}
The first step our graph reordering is to assign nodes to hash buckets based on their neighborhood similarity and enumerate all such pairs. Then, for all such pairs, we apply tree-based clustering algorithm to reduce node pairs into clusters, where nodes inside clusters share the most number of common neighbors. Finally, we reorganize the rows/columns of the adjacent matrix to get the updated adjacent matrix and row/column node ID sequence. 
\end{comment}

\subsubsection{Computation Complexity}
Graph reordering is very lightweight and based on the row and column LSH clustering. LSH has low computation complexity and is friendly for parallel computing. The complexity of the row or column LSH clustering is $O(n*|H|)$, where $n$ is the node number and $|H|$ is the number of hashing functions. For practical use, we can constrain the row and column clustering inside a sliding window. For Citeseer,   


, where one $n$ \abanti{is} for construct \abanti{constructing} the hash table based on the node vector and another $n$ for building the nearest neighbor pairs of each point. Clustering the nodes takes $O(p\log n + (p+n)\log p)$, where $p$ is the node pairs, $n$ is the total number of nodes of the graph. Specifically, searching and inserting the non-cluster-root node pairs takes $O(p\log n)$, merging two clusters takes $(p+n)\log p$. The complexity of the matrix transformation takes $O(n)$, where $n$ is the number of nodes inside the graph.  For the Redit dataset with 232,965 nodes, the graph reordering only requires several seconds (\abanti{'Several' seconds is very vague. What is the exact number?}) to complete, which is practical for preprocessing \abanti{It is pretty well-established that graph reordering can be quite expensive. So, I think reviewers will ask for explicit values of preprocessing times and execution times for all datasets, even if it is claimed that it is very lightweight. Is it possible to provide an explicit tabulation of preprocessing times for all datasets? It is also important to show both preprocessing time AND execution time. This way it is solid evidence that preprocessing is really lightweight}. 




%The adjacent matrix status before each row/column reordering should be safely recorded for backup, as shown at \textit{line 7 and 16}, just in case the proposed row/column reordering is "inferior" (i.e., can not reduce RLE). In each iteration, we first apply row reordering (\textit{line 9}), and evaluate its column-wise RLE (at \textit{line 10}). If the proposed row reordering can effectively reduce the column-wise RLE, we will keep the updated matrix based on the proposed row reordering. Otherwise, we will discard the updated \textit{adjMat} and reset it to pre-reordering status, meanwhile adding 1 to \textit{earlyStop} for potential early termination. The similar reordering process can be applied to column reordering, which spans from \textit{line 18}  to \textit{line 24}, where row-wise RLE is evaluated. At the end of each iteration, we check the \textit{earlyStop}. If \textit{earlyStop} reaches 2, which means both of the proposed row/column reordering fail to reduce RLE in the current iteration, we will set \textit{rowColChange} to False, which will terminate the graph transformation algorithm at the end of current iteration. 
\begin{comment}


\begin{algorithm}[h] \small \label{alg: LSH-based Row/Column Reordering}
\SetAlgoLined
\SetKwInOut{Input}{input}
\SetKwInOut{Output}{output}
\Input{adjMat, sigLen, cluSize, axisSign\;}
\Output{optAdjMat, rowOrder, colOrder\;}
\caption{LSH-based Row/Column Reordering.}

nodePairSimQue = LSH(adjMat, sigLen, axisSign);\\
clusters = nodeClusters(nodePairsSimQue, cluSize);\\
optAdjMat, rowOrder, colOrder = matTrans(clusters);\\
\end{algorithm}

\end{comment}

% \begin{algorithm}[h]
% \SetAlgoLined
% \SetKwInOut{Input}{input}
% \SetKwInOut{Output}{output}
% \Input{adjMat, sigLen, clusterThreshold}
% \Output{OptAdjMat}
% numCluster = numNode - 1; \\
% simQueue = LSH(adjMat, sigLen); \\

% \While{simQueue.size() > 0 \&\& initCluster > 0}{
%     (nodeI, nodeJ) = getHighestSimNodePair(simQueue)
%     rootI, rootJ = getRoot(nodeI), getRoot(nodeJ)
%     \uIf {nodeI == rootI \&\& nodeJ == rootJ}{
%         \uIf {nodeI.clusterSize < nodeJ.clusterSize}{
%             setRoot(nodeI.nodes, nodeJ)
%             \uIf nodeJ.numNodes > clusterThreshold
%                 removed(nodeJ)
%                 numCluster -= 1;
%         }
%         \uElse{
        
%         }
%     }
%     \uElse{
%         \if traversed[rootI] or traversed[rootJ]:
%             continue
%         \uIf{(rootI, rootJ) not in simQueue}{
%             simQueue.insert((rootI, rootJ));
%         }
%     }
    
%     rootJ

% } 
% \end{algorithm}
% \subsection{Mapping Generating}
% \paragraph{Naive Mapping}
% \paragraph{Cache-locality Aware Mapping}
% \paragraph{Node Balance Mapping}

\subsubsection{Reordering Effectiveness.}
We use the length of Run-length Encoding (RLE) as the metric to quantify the effectiveness of reordering. RLE is a sequences\abanti{sequence}-targeted lossless data compression technique: if the same data value occurs in many consecutive data elements, RLE will store a single data value and the count of it, rather than the original data. Taking the example in Figure~\ref{fig: Row-Column Reordering.} for example. In the original graph, the RLE of the column 3 is $1013121$. After row/column transformation, the RLE of the column 3 is $04130$. The length of this RLE code is reduced during transformation process.   
 An effective reordering that can generally offer a smaller value of RLE accumulation, which indicate that the nodes with more shared neighbors will be executed consecutively. Thus the feature data of their neighbors will be reused in the cache with shorter temporal distance. 
 
 \abanti{ Some clarifications are probably best:
 \begin{itemize}
     \item Is run-length encoding a well-known concept or did you invent it? It is necessary to write this explicitly. If it is an old technique, could you cite it? If it is novel, we should boldly write it is a novel technique which has never been applied before.
     \item When is RLE encoding process run? At the end of reordering? During the reordering? If RLE number is poor, what do you do? Stop/Cancel the reordering or still go with it? What is the overhead of RLE? How do you further use the RLE value??
 \end{itemize}
}

%Specifically, to evaluate a row reordering performance, we measure the column-wise RLE, since a successful row reordering can often offer a smaller column-wise RLE. As shown in Figure~\ref{fig: Run-length Encoding.}(a), the column-wise RLE accumulation has been reduce to 19 after the row reordering. Similarly, to evaluate the column reordering, we measure the row-wise RLE accumulation, as shown in Figure~\ref{fig: Run-length Encoding.}(b), the row-wise RLE accumulation of matrix B has been effectively reduce from 21 to 19. An effective reordering that can generally offer a smaller value of RLE accumulation will be kept, whereas the inferior reordering that fail to reduce or even increase the RLE will be discarded.
\begin{comment}
\begin{figure}[h] \small
    \centering
    \includegraphics[width=0.8\columnwidth]{fig/algo-3.pdf}
    \caption{Run-length Encoding.}
    \label{fig: Run-length Encoding.}
\end{figure}
\end{comment}
\begin{comment}
\begin{algorithm}[h] \small \label{alg: RLE encoding.}
\SetAlgoLined
\SetKwInOut{Input}{input}
\SetKwInOut{Output}{output}
\caption{Evaluate Run-length Encoding.}
\Input{adjMat, axisSign\;}
\Output{RLEVal\;}
\caption{Run-length Encoding Evaluation}
RLEList = applyRLE(adjMat, axisSign); \\
RLEval = Accumulate(RLEList);
\end{algorithm}
\end{comment}
\noindent\textbf{Shared Node Set Exploration.}
Based on the reordered graph, we explore the reuse potentiality of the intermediate aggregation results. The basic idea is to find the shared node sets in the window of neighboring rows. In this work, the node set granularity is set to 2 for the simplicity of implementation. The detail is illustrated in Figure~\ref{fig:IA_reuse}, where node 2, node 6 share the neighbor of node 4 and node 5. Therefore, the intermediate results of node4 and node 5 can be reused for node2 and node6 aggregation computation. 

\begin{figure}[!th] \small
    \centering
    \includegraphics[scale=0.45]{fig/aggregration-reuse.pdf}
    \caption{Row-Column Reordering.}
    \label{fig:IA_reuse}
\end{figure}


\begin{comment}
\begin{algorithm}[h] \label{alg: Graph Transformation.} \small
\SetAlgoLined
\SetKwInOut{Input}{input}
\SetKwInOut{Output}{output}

\Input{adjMat, sigLen, cluSize, iterNo\;}
\Output{optAdjMat, rowOrder, colOrder\;}
\caption{Graph Transformation.}

earlyStop = 0\;
rowColChange = True\; 
iterCnt = 0\;
preRowRLE = INF\;
preColRLE = INF\;
\While{rowColChange \&\& iterCnt $\leq$ iterNo}{
    preMat = adjMat\;
    
    // Row reordering \\
    adjMat, rowOrder, colOrder = Reordering(adjMat, sigLen, cluSize, "row")\;
    colRLE = evalRLE(adjMat, "col")\;
    \uIf {colRLE < preColRLE}{
        preColRLE = colRLE\;
    }
    \uElse{
        earlyStop++\;
        adjMat = preMat\;
    }
    preMat = adjMat\;
    
    // Column reordering \\
    adjMat, rowOrder, colOrder = Reordering(adjMat, sigLen, cluSize, "col")\;
    rowRLE = evalRLE(adjMat, "row")\; 
    \uIf {rowRLE < preRowRLE}{
        preRowRLE = rowRLE\;
    }
    \uElse{
        earlyStop++\;
        adjMat = preMat\;
    }
    
    \uIf {earlyStop == 2}{
        rowColChange = False\;
    }
    earlyStop = 0\;
    iterCnt++\;
 }
\end{algorithm}
\end{comment}




==> tex/archDesign.tex <==

\section{\Mname Design }

\subsection{Key Design Concept}
%\Note{three GNN models, ten datasets}

%\Note{Time-breakdown for bottleneck analysis}
%\subNote{Scatter dominants the execution time}
%\subNote{feature size and edge number influence on the bottlenecks}
%\subNote{Relationship between Scatter time and edge size and feature size}
%issues of traversal overhead, heavy computing complexity, and synchronization stall 
To address the challenges in GNNs, we propose the accelerator design based on spatial architectures in harmony with NN accelerators, and optimize for both dataflow of both the Euclidean and non-Euclidean data in GCN processing. analyze the computation of both the Euclidean and non-Euclidean data in GNN processing flows. We observe that there are two types of dataflow during GNN execution: Euclidean data flow inside single node feature computation and non-Euclidean data flow during aggregation reduction among neighboring nodes. %the node reuse is very important to address these issues. 
\textbf{Euclidean data flow inside single node: }
Taking the illustrative case in Figure~\ref{fig:reuse}.a as an example, during the embedding calculation of $node4$, feature extraction and update operations exhibit Euclidean data flow. Thus the spatial architecture can be used to optimize the data reuse in either verizon, horizontal, or diagonal directions~\cite{eyeriss}. 
\textbf{ Non-Euclidean data flow between nodes: }
The aggregation reduction operation, however, involves the graph traversal and computations for non-Euclidean data.  
Specifically, there are two types of data reuse in Aggregation function: input feature data reuse and partial aggregation results reuse. 1) Input feature data reuse: As shown in Figure~\ref{fig:reuse}.b, the feature data of $node$ 2 are repetitively used when conducting neighbor aggregation for $node$ 4, $node$ 1, $node$ 3, and $node$ 5. 2) Intermediate aggregation results reuse: Since the $node$ 4 and $node$ 5 have the shared neibor sets: $node$ 2 and $node$ 6, the intermediate aggregation results of $node$ 2 and $node$ 6 can be reused when computing the aggregation for $node$ 4 and $node$ 5 because the aggregation reduction operations are based on sum, average, or min/max, which are order invariant. Although there are large volume of potential data reuse, it can be hardly handled by the spatial architecture with Euclidean data reuse path, because there is no specific order and geometric data reuse direction for such computations. 




\begin{figure}[h]
    \centering
    \includegraphics[scale=0.32]{fig/data_reuse.pdf}
    \caption{Date Reuse of non-Euclidean Data: 1) feature data reuse; 2) intermediate aggregation result reuse.}
    \label{fig:reuse}
\end{figure}


In summary, GNN computing involves both the Euclidean and non-Euclidean data flow. To achieve efficient GNN computation, we propose an accelerator design to optimize the dataflow of both the Euclidean and non-Euclidean data. 
The high-level block diagram of the \Mname system is illustrated in Figure~\ref{fig:DesignOverview}. 
%\abanti{We propose an accelerator to optimize both Euclidean and non-Euclidean dataflows}. 
Euclidean data can be handled sufficiently well by the spatial architectures~\cite{eyeriss}, which are utilized in the existing DNN accelerators. 
Optimization of the non-Euclidean dataflow, on the other hand, is achieved with the temporal reuse opportunities in the cache hierarchy.  
Furthermore, we propose a lightweight graph ordering and a task mapping methodology to improve the cache access efficiency and alleviate the workload imbalance issue. The accelerator design details are introduced in the following. 
\begin{figure*}[h]
\centering  
\includegraphics[scale=0.50]{fig/overview.pdf}
\caption{Design Overview.}
 \label{fig:DesignOverview}
 
\end{figure*}

%For the neural network computing operations inside every node (feature extraction and update), the data is reused within the register files of MAC array. For the non-Euclidean data flow during aggregation reduction, the data is reused temporally in PE cache 



%\abanti{we dedicated one line to explain synchronization. I think we should also dedicate one line to workload imbalance for fairness purposes}
%Workload imbalance occurs when some node have much more neighbors than the others. 

\begin{comment}
\textbf{Micro-instructions generation:} The micro-instructions generated for three main processing functions in GCNs, feature extraction, aggregation, and update, are illustrated in (\todo{one illustrative figure}). To compute the hidden status of node 1, the micro-instructions are as follows: first load the node feature data of its neighbors (line1-line3: load node2, load node3, load node4). Then compute the aggregation function (compute aggregate(node2, node3, node4)). Store the aggregation results (store aggregate(node2, node3, node4)). Such processing steps are iteratively conducted for every node in the graph and finally compute the update function (compute update(aggregate)).
\todo{Need Xinfeng's help}
\end{comment}


\subsection{Accelerator }

The architectural design of \Mname is demonstrated in Figure~\ref{fig:DesignOverview}.  \Mname is mainly comprised of
of the following basic components: processing element (PE) array, memory controller, global on-chip buffer, and control logic. 
%The traversal engine implements the efficient graph traversal, constructs and reorders the computational graphs, and schedules the tasks to the PE arrays. 
The PE array performs feature extraction, aggregation reduction, and update operations. 
The on-chip buffer stores the data shared by the whole PE array, such as the weight matrices of graph convolutional network. 
We describe next the design details of these components and the data reuse strategy in \Mname. 

\begin{comment}
\subsection{Traversal Engine}
\subsubsection{Graph Traversal}
\subsubsection{Graph Reordering}
\subsubsection{Task Mapping}
\end{comment}


\subsubsection{PE Array}
The PE array consists of multiple PEs connected with 2D-mesh network on chip (NoC) interconnections. The leftmost and rightmost PEs in the NoC mesh communicate with memory controller directly. The other central PEs get the read and send write requests through the 2D-mesh NoC. All the traffic between PEs and memory goes through the NoC network in a first come and first service manner with one way routing strategy. Specifically, there are two memory controllers in \Mname at the left and right side of PE arrays. The access location of a memory request is determined by the memory address. Once the access location is determined, the memory request is transferred through the NoC at either left-horizontal or right-horizontal directions.  
  
The detail design of PE is shown in Figure~\ref{fig:DesignOverview}(c), which consists of the instruction queue, the load-store queue (LSQ), the NoC queue, the  multiply and add accumulator (MAC) array, and two private caches for data reuse of non-Euclidean data. 
%node feature and intermediate aggregation results buffering. 
Instruction Queue buffers the micro-instructions including three major categories: load; store; and computation. The entire GNN training process can be translated to hardware primitives according to the input graphs.  The micro-instructions can be generated by the driver and prefetched to the instruction queue with streaming strategy for good access efficiency. LSQ buffers the load and store requests for accessing the feature extraction data, aggregation data, and update data. 

\subsubsection{On-chip Memory Hierarchy}
Hierarchically, the on-chip memory consists of several layers which handle different data reuse granularities: global buffer, PE private cache, and MAC register files (RFs).
Global buffer: Global buffer exploit data reuse between PEs such as the weight matrices. PE private cache buffers the feature map data and intermediates aggregation data for input reuse and partial sum reuse of non-Euclidean data  in Figure~\ref{fig:reuse}. Such data reuse is in temporal manner based on the cache implementation. Tasks in different PEs do not have non-Euclidean data reuse in these private cache. Thus, during task mapping, we should carefully do the tradeoff between task parallelism and data reuse efficiency. 
MAC register files are similar like that in neural network accelerators which exploit all types of data movement within the computations of one node, including the convolutional reuse, ifmap reuse, and filter reuse.  
Except the weight metrics, all other store requests are write-through and sent back to the memory controller directly without on-chip buffering. 



\subsection{Programming Model and Hardware Primitives}
To generally support diverse graph neural network algorithms, we adopt a vertex-centric programming model, since most graph neural network are based on this model~\todo{ref}. Based on the vertex-programming model, we provide the following hardware primitives to support the execution of GCNs in  Algorithm~\ref{alg:gcn}: \textit{load-f}, \textit{load-i}, \textit{comp}, and \textit{store}. 
The first two primitives, \textit{load-f} and \textit{load-i}, are used to load and aggregate the feature vector of single node and the intermediate aggregation result of two nodes. 
The third primitive, \textit{comp}, is used to invoke the computation of feature extraction and update function, which is usually composed to matrix-vector multiplication and some element-wise computation instructions.
After computing the feature vector of a node $v$ for the $k$-th layer ($h_v^{(k)}$), the \textit{store} primitive is used to flush the result of computation into memory so that it is visible to other PEs in the iteration of $(k+1)$-th layer.


Vertex-centric programming models are confronted with synchronization issues during execution, overhead of which is introduced when the node update operation is blocked due to waiting for the neighbors to be aggregated. Thus, we propose graph reordering method and intelligent mapping to alleviate irregular memory access effect and reduce synchronization overhead, while retain the task-level parallelism. 
The graph reordering and mapping stage generates two inputs to hardware accelerator. The first input is the task assignment with the ordered vertex ID.
In particular, each PE is assigned with a set of vertices to compute (from line 5 to 10 in Algorithm~\ref{alg:gcn}).
The second input is the indicator for reuse of the intermediate aggregation results, which generates the \textit{load-i} instructions. 
%reorder for traversing the neighbours of a vertex $v$ (from line 6 to 8 in Algorithm~\ref{alg:gcn}).
%This input of traversing sequence also indicates whether the access to the feature vector of neighbour vertices is a \textit{load-f} (feature data) or a \textit{load-i} (intermediate aggregation results).
The hardware accelerator executes these hardware primitives generated by the reordering and mapping stage, and the reordering and mapping stage is responsible to exploit the locality of feature vectors and the computation reuse of partial intermediate results.

\subsection{Task Mapping}
Graph reordering 
\noindent\textbf{Mapping to PEs.}
The mapping strategy of allocating vertexes to PEs considers both data reuse and task-level parallelism. 
In the adjacency matrix of transformed input graph, the destination nodes of neighboring rows have the similar source nodes for aggregation, which introduces both the input data reuse and intermediate aggregation result reuse. To improve the data reuse along their execution, we evenly partition the rows to 64 sets (the number is equal to that of PE number). Then allocate every set to an individual PE for parallel computation. Such process is illustrated in Figure~\ref{fig:DesignOverview}.

\noindent\textbf{Mapping to MAC Array}
For the feature computation inside nodes (feature extraction and update), we tile the vector matrix multiplication onto the MAC arrays. Such mapping, tiling, folding methodology have been studied in previous neural network accelerators. We adopt the similar methodology, as shown in Figure~\ref{fig:reuse}.





\subsection{Computation Process}

\begin{figure*}[h]
\centering  
\includegraphics[scale=0.55]{fig/dataflow.pdf}
\caption{Data reuse.}
 \label{fig:dataflow}
 
\end{figure*}


As introduced in Section2, the whole processing pipeline of forward propagation is comprised of feature extraction, aggregation reduction, and update. The detail forward propogation computation and dataflow are shown in Figure~\ref{fig:dataflow}.

In summary, the data reuse in \Mname can be generally classified into two categories: reuse of non-Euclidean data and Euclidean data. For the computation inside a node (Euclidean data), such as feature extraction and update stages, the feature map data and weight matrix are reused in MAC arrays. For the computation on the node set for aggregation (non-Euclidean data), the feature data is stored in the private cache of every PE for temporal reuse. 

\noindent\textbf{Feature Extraction.} Feature extraction for nodes is conducted at the begining of every iteration. During this process, the feature data of nodes are streaming in and streaming out to memory systems. Weight data is stored onto the global buffer and reused for the feature extraction of every node. 

\noindent\textbf{Aggregation Reduction.}
After the completion of feature extraction, \Mname conducts aggregation reduction for every node, by loading and computing the feature data of its node neighbors. The feature data is buffered in private cache of PE. Along the aggregation for the nodes in the input graph, there is temporal reuse of feature map data in the private cache after the graph reordering. Such temporal data reuse reduces off-chip memory accesses and the Section 6.4 discussed the effect with quantitatively analysis. Specifically, there are two types of reuse: 1)  the feature data of every node, which is the input of aggregation reduction function, is stored in S-Cache. 2) The intermediate aggregation results of node sets, which are stored in A-Cache. For the graphs with large degrees, A-Cache is helpful to reduce the computations of aggregation  significantly. 

\noindent\textbf{Update.}
With the aggregation results of a node, the update operation is conducted which calculate with the input of the aggregation results and the weight metrices. During the node computation, the weight data and feature data are reused in MAC arrays and the global buffer. The final result of the updated feature data will be written through to off-chip memory directly. 







\begin{comment}
\subsubsection{Computing}
\noindent\textbf{Node Feature Computation.}

\noindent\textbf{Localized Reduction.}

\end{comment}



%\subsection{Task Mapping}






==> tex/biography.tex <==
\vspace{-40pt}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{fig/photo/xinghu}}] {Xing Hu} received the B.S. degree from Huazhong University of Science and Technology, Wuhan, China, and Ph.D. degree from University of Chinese Academy of Sciences, Beijing, China, in 2009 and 2014, respectively. She is currently an associate professor of State Key Laboratory of Computer Architecture, Institute of Computing Technology (ICT), Chinese Academy of Sciences (CAS), Beijing, China. Her current research interests include emerging memory system and domain-specific hardware computing.
She publishes over 30 papers in major conferences and journals including MICRO, HPCA, ASPLOS, DAC, DATE, TCAD, TVLSI, TACO, etc. She serves as reviewer for a number of journals and conference.
\end{IEEEbiography}
\vspace{-40pt}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{fig/photo/yukewang}}] {Yuke Wang} received his B.E. degree from the University of Electronic Science and Technology of China (UESTC), Chengdu, China, in 2014 and 2018. He is currently pursuing the Ph.D. degree at Department of Computer Science, University of California, Santa Barbara (UCSB), USA. His current research interests include graph neural network and its acceleration on CPUs, GPUs and FPGAs. 
\end{IEEEbiography}
\vspace{-40pt}

\begin{IEEEbiography}[{\includegraphics[width=1in, height=1.25in, clip, keepaspectratio]{fig/photo/leideng}}] {Lei Deng} received the B.E. degree from University of Science and Technology of China (USTC), Hefei, China in 2012, and the Ph.D. degree from Tsinghua University (THU), Beijing, China in 2017. He is currently a Postdoctoral Fellow at the Department of Electrical and Computer Engineering, University of California, Santa Barbara (UCSB), CA, USA. His research interests span the area of brain-inspired computing, machine learning, neuromorphic chip, computer architecture, tensor analysis, and complex networks. He has authored over 30 publications. He serves as a Guest Associate Editor for \emph{Frontiers in Neuroscience} and \emph{Frontiers in Computational Neuroscience}, a PC member for \emph{ISNN} 2019, and a reviewer for a number of journals and conferences.
\end{IEEEbiography}
\vspace{-40pt}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{fig/photo/lingliang}}] {Ling Liang} received the B.E. degree from Beijing University of Posts and Telecommunications, Beijing, China, in 2015, and M.S. degree from University of Southern California, CA, USA, in 2017. He is currently pursuing the Ph.D. degree at Department of Electrical and Computer Engineering,  University of California, Santa Barbara, CA, USA. His current research interests include machine learning security and computer architecture.
\end{IEEEbiography}
\vspace{-40pt}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{fig/photo/pengfeizuo.jpg}}] {Pengfei Zuo} Pengfei Zuo received the BE degree in computer science and technology from Huazhong University of Science and Technology (HUST), China, in 2014. He is currently a PhD student majoring in computer science and technology at HUST and a visiting PhD student at UCSB. His current research interests include non-volatile memory, storage systems and techniques, and memory security. He publishes several papers in major conferences and journals including OSDI, MICRO, USENIX ATC, SoCC, ICDCS, IPDPS, MSST, DATE, TPDS, TOS, TCAD, etc. He is a student member of IEEE.
\end{IEEEbiography}
\vspace{-40pt}


\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{fig/photo/yejing.jpg}}]{Jing Ye}
Ye Jing is currently an associate professor of State Key Laboratory of Computer Architecture, Institute of Computing Technology (ICT), Chinese Academy of Sciences (CAS), and an assistant secretary-general of Technical Committee on Fault Tolerant Computing, China Computer Federation. He received the Ph.D. degree in ICT, CAS in 2014, and the B.S. degree in Electronics Engineering and Computer Science, Peking University in 2008. His current research interests include VLSI test, hardware security (physical unclonable function, hardware Trojan, etc.), and AI software/hardware security.
\end{IEEEbiography}
\vspace{-40pt}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{fig/photo/Yingyan_journal}}]{Yingyan Lin} received her Ph.D. degree in electrical and computer engineering from the University of Illinois at Urbana-Champaign (UIUC) in 2017. Since Fall 2018, she has been an Assistant Professor in the Department of Electrical and Computer Engineering at Rice University. She is currently leading the Efficient and Intelligent Computing (EIC) Lab at Rice, which is exploring techniques to enable powerful yet complex machine learning systems to be deployed into resource-constrained platforms. 

She served as a session chair of ISCAS 2019 and ICCAD 2018, and is currently in the TPC of DAC 2020, MobiCOM 2020, SECON 2020, and NeurIPS 2020. Her current research focuses include efficient machine learning algorithms, efficient machine learning acceleration architectures, and algorithm-hardware co-design for energy/time-efficient machine learning systems.
% embedded machine learning, i.e., developing  energy/time-efficient machine learning systems for resource-constrained platforms.


% She received a Best Student Paper Award at the 2016 IEEE International Workshop on Signal Processing Systems (SiPS 2016) and the 2016 Robert T. Chien Memorial Award at UIUC for Excellence in Research, and was named a Rising Star in EE/CS by Stanford University in 2017. Her current research focus is embedded machine learning, i.e., developing  energy/time-efficient machine learning systems for resource-constrained platforms.

\end{IEEEbiography}
\vspace{-80pt}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{fig/photo/yuanxie}}]{Yuan Xie}  received his Ph.D. degrees from Electrical Engineering Department, Princeton University, Princeton, NJ, USA in 2002. He was with IBM, Armonk, NY, USA, from 2002 to 2003, and AMD Research China Lab, Beijing, China, from 2012 to 2013. He was a Professor with Pennsylvania State University, State College, PA, USA, from 2003 to 2014. He is currently a Professor with the Department of Electrical and Computer Engineering, University of California at Santa Barbara, Santa Barbara, CA, USA. 

Dr. Xie is an expert in computer architecture who has been inducted to ISCA/MICRO/HPCA Hall of Fame. He has been an IEEE Fellow since 2015. He served as the TPC Chair for HPCA 2018 and he is Editor-in-Chief for ACM Journal on Emerging Technologies in Computing Systems (JETC), Senior Associate Editor (SAE) for ACM Transactions on Design Automations for Electronics Systems (TODAES), and Associate Editor for IEEE Transactions on Computers (TC). His current research interests include computer architecture, Electronic Design Automation, and VLSI design.
\end{IEEEbiography}

==> tex/design.tex <==
\section{Characterization and Motivation}
%\todo{Xing}
%\abanti{In this section, we quantitatively characterize GCN workloads and provide insights on how they differ from graph computing and neural networks in terms of unique challenges. In addition, we highlight the dual dataflow in GCNs which is a key motivator for our accelerator design. }

In this section, we quantitatively characterize GCN workloads and provide insights on how they differ from graph computing and neural networks and their unique challenges. And we also highlight the hybrid computing paradigm and dual dataflow in GCNs, which is a key motivator of our accelerator design.






%\subsection{Comparisons with NN and Graph}
 %GCN computing paradigm combines both the computing models of graph and neural networks. Therefore, we compare GCN with graph computing and neural networks in terms of its compute complexity and dataflow, correspondingly. At last, we provide guidelines for architectural-level optimizations of GCN accelerator designs.
 %\abanti{We compare GNN with graph computing and neural networks, focusing on compute complexity and dataflow. Finally, we provide guidelines for architectural-level optimizations.}
 
\subsubsection{GCN vs. NN}
%used for classification, regression, or even reasoning. Taking convolutional network as an example, it is
The node-level computing in GCN is similar like NN which operates on the regular Euclidean data like images or text to obtain the highly expressive representations. 
%They are commonly constructed with multiple convolutional, activation, and fully-connected layers sequentially stacked together. 
%, which extracts multi-scale spatial features and obtains the highly expressive representations, as shown in Figure~\ref{fig:gnn_comparison}.a. 
%CNNs operate on the regular Euclidean data like images or text.  
The graph-level computing in GCNs, however, operate on non-Euclidean data of the input graphs, which introduces the graph traversal overhead.
\xing{move something to basics}

\xing{in this section, we should deliver the messages: 
1) various demands with different graphs and graph algorithms.
2) various 
Two types of data reuse: graph level, node level in three phases, extraction, aggregate, update}

%, incorporating the concepts of both graph computing and deep neural networks. %As introduced in Section 2.2, the GCNs exhibit the graph computing mode that aggregates the node representations from the neighborhood, and the neural network computing mode that extracts and embeds the features or hidden states of nodes/edges/subgraphs with deep neural network techniques. 
%Thus, GCNs differ from NNs in the additional graph traversal overhead. 
We conduct the execution time breakdown of GraphSage~\cite{GraphSage} forward propagation on GPU platform over six datasets, as shown in Figure~\ref{fig:graphsage_breakdown}. The details of these datasets are presented in Section~\ref{sec:setup}. The results show that 1) Graph-level computing (\emph{Aggregation}) exhibiting graph traversal occupies a large proportion of the overall execution time. 2) Diverse workloads (\textit{e.g.}, Citeseer-S vs. Reddit) with different feature size and graph scale have different bottleneck of graph-level computing (\emph{Aggregation}) or node-level computing (\emph{Update}) . 
%\todo{Comparison between euclidean and non-euclidean dataflow }
\begin{figure}[!htbp]
    \centering
    \includegraphics[scale=0.55]{fig/breakdown_sage.pdf}\vspace{-10pt}
    \caption{Execution time breakdown of GraphSage: Aggregate vs. Update.}
    \vspace{-0.6em}
   \label{fig:graphsage_breakdown}
\end{figure}

Graph-level computing could bring two challenges:
\noindent\textbf{Irregular memory accesses.} Graph traversal during the aggregation of the feature data of neighboring nodes introduces a large volume of irregular memory accesses. 
This is in contrast to NNs on Euclidean data where the memory access patterns are hardware-friendly because it can be regularly transformed to matrix/tensor computations.
%Irregular memory accesses bring large memory overhead. When computing the Euclidean data in DNNs, the memory access and processing pattern are hardware friendly because it can be regularly transformed to matrix/tensor computations. 
%In GCNs, however, graph traversal during aggregating feature data of neighboring nodes introduces larger volume of irregular memory accesses. 
Hence, GCNs are more memory-bounded compared to NNs.
This is further confirmed by our VTune analysis in Figure~\ref{fig:comparison}.
%, according to the Vtune analysis~\cite{Vtune}. As illustrated in Figure~\ref{fig:comparison}
NNs execution are more dominated by their computations. 
The smaller networks, such as Lenet, are mainly computing bound. 
The larger networks, such as ResNet18 and VGG19, have more memory stall time because of the larger weight and feature map matrices. Thus, lots of data flow optimizations are proposed to enlarge data reuse and eliminate the off-chip memory accesses~\cite{eyeriss}. However, such data reuse methodologies are not applicable to GCN graph-level computing which conducts computations on non-Euclidean data with irregular memory accesses. \textbf{Synchronization stalls.} Synchronization stalls are introduced by irregular memory accesses. % and workload imbalance inherited from the irregularity in graph traversal. 
%is another part of overhead which neural network execution does not have. 
Specifically, in \emph{Aggregate} function, all the feature data of in-neighbors during graph traversal should be in ready status before conducting the aggregation reduction operations. 
If the feature data of one neighbor misses, the aggregation function needs to wait even when all the other neighbor feature data is ready in the cache.
Therefore, the synchronization among neighbors is another key source of the computation overhead. Such synchronization contributes to the computation stalls in Vtune analysis in Figure~\ref{fig:comparison}.
% \vspace{-2em}
\begin{figure}[!t]
    \centering
    \includegraphics[scale=0.50]{fig/overall_breakdown.pdf}\vspace{-10pt}
    \caption{Stall breakdown of Graph, NN, and GCN applications.\protect\footnotemark}
    \label{fig:comparison}
\end{figure}

\subsubsection{GCN vs. Graph}
Graph analytics possesses a similar programming model as the graph-level computing in GCNs. As shown in Figure~\ref{fig:gnn_comparison}, in a pull-implementation programming model of graph computing, processing a vertex involves three steps: 1) \emph{Gather}: reading properties from the in-neighbors of vertex; 2) \emph{Apply}: processing the update operation on the gathering properties. The functionalities of \emph{Gather} and \emph{Apply} are similar to \emph{Aggregate} and \emph{Update} operations in GCNs. However, at the node-level computing, GCN and graph analytics have different data dimensions and computation complexities of nodes/edge features, as compared in Table~\ref{tab:gnn_graph}.
%\abanti{In every enumaerated point, it is important that we explain a supporting data, not just the observation}. 
GCNs, in general, have much larger feature data size (10x -- 1000x) than the property data in graph analytics applications. In addition, \emph{Aggregate} and \emph{Update} operations in GCNs have significantly larger computation complexity due to neural network computing, while that in graph analytics usually consist of simple scalar computations. 
%2) For every node, there is no feature extraction on the property data in graph computing, while GNNs have.
%3) Aggregation and update functions in graph computing are based on scalar data, while that in GNNs are based on large vectors.
%4) Both feature extraction and update in GNNs involve the neural network computing which are much more computing-intensive than the simple functions in graph computing. 
%\abanti{
%Just a comment: The differences between Graph and GNN that you point out, I would not say these observations are derived from "explicit characterization". The table is a tabulation of very qualitative and common sense things, not the observations derived from some quantitative measurement. So,
%maybe this section should be in background?? }
%However, the data scale and computation complexity of node/edge make the GCN significantly different from the graph neural networks. We compare several important metrics as follows. 




% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\caption{\label{tab:gnn_graph}{Graph Computing vs. Graph Neural Network.}}
 \scalebox{0.7}{
\begin{tabular}{|c|c|c|c|c|}
\hline
\multirow{2}{*}{} & \multicolumn{2}{c|}{\textbf{Graph Computing}} & \multicolumn{2}{c|}{\textbf{Graph Neural Network}} \\ \cline{2-5} 
 & SSSP & PR & Citeseer & Reddit \\ \hline
\begin{tabular}[c]{@{}c@{}}Property/Feature\\ Size\end{tabular} & 4Bytes & 4Bytes & 3703*4Bytes & 602*4Bytes \\ \hline
Feature Extraction & / & / & DNN & DNN \\ \hline
Aggregate & Scalar & Scalar & \begin{tabular}[c]{@{}c@{}}Vector Reduction\\ (1024/128)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Vector Reduction\\ (1024/128)\end{tabular} \\ \hline
Update & Scalar & Scalar & DNN & DNN \\ \hline
\end{tabular}}
\vspace{-1.5em}
\end{table}

Because of the different data dimensions and processing complexity, graph analytics and GCNs exhibit different bottlenecks at the architecture level. 
First, graph applications are mainly memory-bound because of the irregular accesses and simple update computation~\cite{abanti_hpca}, whereas GCNs demand more computation capabilities. 
%As shown in Figure~\ref{fig:comparison}. 
Second, typical prefetch-oriented optimizations in graph analytics (\textit{e.g.}, prefetching property data on to on-chip buffers for better memory access efficiency) are less effective in GCN applications. This is because less node feature data can be prefetched than that in graph analytics due to the larger feature data size (hundreds to thousands of times larger than property data in graphs). 
%In addition, the computation of feature extraction and update (NN computing) involves lots of intermediate data with regular memory accesses. Such regular and irregular memory accesses interact with each other and prefetching may have negative impacts on the cache performance.
%\abanti{In addition to prefetching, there are other techniques used for traditional graphs such as hardware-accelerating traversals, acceleration of worklists. Do we need to mention them? Second, do we have a reference which proves that prefetching in the presence of both regular and irregular memory access has side effects?}. 
In summary, GCN is confronted with the following challenges:  irregular memory accesses and synchronization overhead introduced in graph-level computing; larger computational complexity in node-level computing. This motivates our accelerator design. 

%\Note{Two indications}
%\subNote{caching or prefetching may have the side effect on cache performance}
%\subNote{The caching overhead for single node is large, and the reuse distance is much longer than Graph applications}


%To understand the difference between GNN, Graph, and NN, we first use Vtune~\cite{Vtune} to analyze the execution bottlenecks of these three categories of applications. 
%For graph workload, two graph analytic applications in the {GAP} Benchmark Suite~\cite{GAP} including Single Source Shortest Path (SSSP) and Pagerank (PR) are profiled using the LiveJournal (LJ)~\cite{LiveJournal} dataset.  For neural network workload, three neural network models in different scales are selected and evaluated based on Cifar10 dataset~\cite{cifar10}, including Lenet~\cite{lenet}, VGG19~\cite{vgg}, and ResNet18~\cite{resnet}. For graph neural network workload, we adopt one commonly-used graph convolutional network, GraphSage~\cite{GraphSage}, on COLLAB graph dataset~\cite{collab}. 

%The overall breakdown is as shown in Figure~\ref{fig:breakdown}. We have the following observations: 1) Graph applications are mainly dominated by memory bound stalls. For SSSP and PR execution, more than 50\% of stalls are incurred by the memory accesses. According to the characterization in Previous work~\cite{Abanti_HPCA}, there exist large volume of load-load dependency in graph applications during graph traversals. 2) Deep neural Network execution is more dominated by computing. The smaller networks, such as Lenet, are mainly computing bound. The larger networks, such as ResNet18 and VGG19, the memory stall time becomes larger because of their larger weight and feature map matrices. However, for deep neural network, lots of previous studies are proposed to optimize for the data reuse to eliminate the memory access problem. Deep neural network is still a computing-bound problem.  3) GCN is bounded by both memory and computation. Compared to Graph, xxx










\begin{comment}
\textbf{Non-Sampling}
\begin{equation}
\begin{aligned}
\scriptsize
#IrregularAccess (bytes) = #Edge * FeatureElementSize, \\
#RegularAccess (bytes) = #Offset * OffsetSize + #Edge * #EdgeSize, \\
 + #Edge * FeatureVectorSize * FeatureElementSize. 
\end{aligned}
\end{equation}

\textbf{Sampling}
\begin{equation}
\begin{aligned}
\scriptsize
#IrregularAccess (bytes) = #SampledEdge * FeatureElementSize, \\
+ #SampledEdge * #EdgeSize, \\
#RegularAccess (bytes) = #Offset * OffsetSize + #SampledEdge * #EdgeSize, \\
+ #SampledEdge * FeatureVectorSize * FeatureElementSize. 
\end{aligned}
\end{equation}
\end{comment}




%\Note{Classify the data in Graph Neural Network into two catogories with different data reuse strategy} \subNote{ 1) Euclidean data flow inside single node.  Spatical architecture for data reuse. }
%\subNote{ 2) Non-Euclidean data flow Temporal architecture for data reuse. }
\begin{comment}
We take the aggregation function in forward-propagation as an example. The processing flow of  backward-propagation is in a similar but reverse way. The aggregation function can be decoupled into two phases: feature extraction and aggregation reduction operation. The input graph for a GCN is as shown in Figurexxx, the processing flow of conducting the aggregation operation for $node1$ is as follows:
1) calculate the feature extraction results of in-neigbhors of node1: f(node2), f(node5), f(node6). 2) aggregate reduction operations: a(f(node2), f(node5), f(node6)). 

Node reuse in this work comprises of both the node feature extraction reuses and nodes aggregation computation reuse. 
node feature extraction reuses: f(node2) will be reused for both node1 and node4.
nodes aggregation reuse: the intermediate aggregation results of f(node2) and f(node5) can be reused by node 4 when it conducts the aggregation function of node2, node5, and node3. We observe that graph ordering is important for the graph neural networks to leverage node reuse for eleminating the irregular memory accesses and the corresponding synchronization stalls. We compare the node reuse distance under two scenarios: sequantial execution and the ordering exeuction in Figure xxx. Graph ordering is an important technique in graph computing, which schedules the execution oerder of graphs without changing the graph algorithms, aiming to improve the cache locality. For graph neural network, the longer reuse distance will results in much more cache misses. Prefetch may be less effective in GCN computing than that in graph computing because of the larger vertex features. Therefore, this work, we propose an efficient ordering algorithm and hardware accelerator to improve the node reuse during GCN computing, which addresses the irregular memory access and the synchronization overhead problems.   
\end{comment}

%. Graph ordering is an important technique in graph computing, which schedules the execution oerder of graphs without changing the graph algorithms, aiming to improve the cache locality. For graph neural networks, the graph ordering is even more important, because of the larger vertex features ( Prefetching is less effective under such cases). Second, graph neural networks tend to learn the nodes with more degrees, which bring significant benefits for training convergence. 







%Data flow in forward-propagation: Two type of node reuses:
%feature extraction data reuse;
%aggregation data reuse;
%Larger data granularity increase the data reuse distance and damage the cache hit rate.
%Goal: ordering to improve the data reuse.
%The dataflow in the backward-propagation is similar. 

\begin{comment}
\Note{Architecture breakdown}
\subNote{L3 Cache miss rate comparison: 1) scatter and combine in the same dataset; 2) miss rate in different dataset with different dimension}
\subNote{CPU ultilization comparison}
\end{comment}

%\Note{Motivation: Node data reuse and compute reuse}
%\todo{A figure to illustrate what is the reuse?}
%\todo{A figure: show how large proportion of the nodes will be reused.}

%\subNote{graph reordering is more important in GNN}
%\subNote{Conclusion: we should consider both the data reuse and computation reuse during accelerating GNNs}



\begin{comment}
\section{Accelerator Design}

\section{Mapping and Scheduling Optimizations}
\subsection{Graph Tiling/Partitioning Strategies}

\subsection{Data Flow Management}

\subsection{}
\subsection{Performance model}
\subsection{Three Design knobs: }
1) Computation Redundancy Elimination; 2) Data Reuse Flow; 3) Task Execution Parallelism




\section{Optimization}

\subsection{Memory-access-friendly Sample}

\textbf{Uniform sample(more irregular memory access).}
Random sample $n$ neighbors in edge list of a node.

\textbf{Sequential sample(more opportunity to access sequentially (high row buffer hit) and reduce the requirement of cache since only a portion of node's feature needs to read to cache).}
Sample $n$ consecutive neighbors in edge list of a node.

Method: find max dense sub-graph (calculate the degree and rebuild edge list) dependent on sample ratio. 

\end{comment}










==> tex/intro_backup.tex <==
\section{Introduction}
With rich and expressive data representation, graphs demonstrates their applicabilities in various domains, such as E-commerce~\cite{RW-GCN,e-business_1,recommendation_gnn}, computer vision~\cite{vision_gnn1,vision_gnn2},  and molecular structures~\cite{molecular}, and \textit{etc}. To fully exploit the their value, approaches based on traditional graph analytics algorithms (e.g., BFS, SSSP) facilitate in-depth understanding of objects-wise relationships in graphs (\textit{e.g.}, molecule similarity in chemistry~\cite{molecular}, cells structures in bioinformatics~\cite{survey_gnn,GNN_Review}, and parsing an image to semantic graphs~\cite{vision_gnn2,vision_gnn1}).  
%For the ease of , graph embedding provides an effective yet efficient way to solve the graph analytics problem. Specifically, graph embedding converts a graph into a low dimensional space in which the graph information is preserved. By representing a graph as a (or a set of) low dimensional vector(s), graph algorithms
Recently, as a raising star, extending deep learning techniques to graph analytics has gained lots of attention from both research~\cite{GraphSage,1stChebNet,FastGCN,DIFFPOOL} and industry~\cite{AliGraph,googleGraph}, largely because of their striking success on Euclidean data (\textit{e.g.}, images, videos, text, and speech). Moreover, such geometric deep learning techniques based on graph neural networks (GNNs) not only learn the inductive representations for end-to-end tasks such as classification, clustering, and recommendation, but also show much better accuracy (more than 98\%) than traditional methods~\cite{RW-GCN} (\textit{e.g.}, random walks~\cite{deepwalk}, and matrix factorization~\cite{survey_graph_embedding}). 
%Impressed by the capability of capturing the hidden representations of Euclidean data, researchers apply that DNN techniques for graph  applications with non-Euclidean data to learn the inductive representations for end-to-end tasks such as classification, clustering, and recommendation. Such geometric deep learning based on graph neural networks (GNNs) shows its good accuracy compared to the traditional techniques including random works or matrix factorization~\cite{RW-GCN}. 
% \st{Thus GNNs become increasingly important nowadays, with contributions from both academia~\cite{GraphSage,1stChebNet,FastGCN,DIFFPOOL} and industry~\cite{AliGraph,googleGraph}.} 
 \begin{figure}[!htbp]
    \centering
    \includegraphics[scale=0.35]{fig/GNN_comparison.pdf}\vspace{-10pt}
    \caption{Graph, GNN, and NN.}
    \label{fig:gnn_comparison}
\end{figure}

Among diverse GNN algorithms and models~\cite{GraphSage,Adaptive_Sampling}, graph convolutional network (GCN) is the most fundamental and have been widely studied. Different GCNs can be summarized and abstracted into a uniform computing model with two stages: \textit{aggregate} and \textit{update}.
% In this work we focus on the most important one, 
%in also have their potentiality for non-Euclidean data which are represented in the form of graphs. Graph neural networks (GNNs) have been become increasingly important in nowadays.  
%====\Note{GNN algorithm works. the uniform abstraction of computing model.}
%GC
\textbf{\emph{Aggregate}} stage collects the localized node representations from the neighboring nodes through two operations: 1) the \textit{feature extraction} for a single node and 2) the \textit{feature reduction} among neighboring nodes.  
The \textbf{\emph{Update}} stage updates the representation vector based on the aggregation results and its previous state. As shown in Figure~\ref{fig:gnn_comparison}, GCN distinguishes itself by combining graph analytics and neural network computing scheme, where the feature extraction and update involve neural network computation while the feature reduction is  essentially a graph traversal. In summary, the GCNs computing is confronted with the following challenges:

1. Hybrid computing paradigm makes the existing NN accelerator and graph accelerator designs pale in effectiveness for handling GCN computing. Since NN accelerators aim to build spatial architectures for powerful computation capabilities while maximizing spatial data reuse~\cite{eyeriss, diannao}. On the other side, graph accelerators prefer resource-intensive on-chip cache to suppress irregular accesses~\cite{graphicionado}. Therefore, an off-the-shelf solution to effectively accelerate GCNs is still missing. And there are two major challenges.
% GCN computing possesses unique features distinguishable from either, which translates to unique  challenges.
%\abanti{There is some problem with the following two lines: in first line, it is mentioned that GNN = graph + DNN. Immediately, in the next line, we say GNN is different from either. My suggestion is below. You can choose which way you like best}.
%\abanti{Although, GNN may intuitively appear to be a combination of graph analytics and DNN, it possesses unique features distinguishable from either, which translates to unique architecture-level challenges. Thus, existing graph or neural network accelerators are inadequate for GNNs.}
% With different feature dimensions and degree distribution, its behavior shifts towards to graph analytics or CNN computing. 
% CNN 
% Thus, existing graph or neural network accelerators are inadequate for GCNs.
%In summary, GNN incorporates both the computing model of graph and DNN techniques. 
%They exhibit the graph computing model which extracts the localized features among neighboring nodes and the neural network computing model that extracts or embeds the features  hidden states of every node. 
%However, GNNs possess unique features distinguishable from either graph analytics or DNN, which makes existing graph or neural network accelerators inadequate for GNNs.  
%As graph data are often irregular with variable node size and complex topology, some important operations (e.g., convolutions) being easy to compute in the image domain, but difficult to apply to the graph domain.
%\Note{Existing accelerators and conclude they are not good enough for GNNs}
%====\todo{Comparison between graph and GNN, and DNN}.


%\todo{Both the challenges and proposed methods (i.e., our contribution) should be well aligned with our key technical sections: Accelerator, Programming Model and Hardware Primitives, Task Mapping Generation... The challenges focus on why we need these components, while the proposed methods center around the key insights (not technical details) behind how we overcome these challenges. The final contribution bullets would include several key proposed techniques (i.e., the subsection titles) in each key technical sections. }

\textbf{Neither NN accelerator and Graph accelerator can handle the hybrid computing paradigm in GCNs efficiently.} 

\textbf{Diverse graph datasets shift the}

\textbf{First, data irregularity and input diversity for localized computation among neiboring nodes.} GCNs localized computing (aggregation reduction) is based on non-Euclidean graph data, which is non-ordered with diverse range of node sizes and topology. 
1) Non-Euclidean data introduces irregular memory accesses and synchronization overhead. 2) Non-Euclidean data cannot be easily handled by spatial architectures for spatial data reuse. 
3) Graph irregularity with variable node volume and feature size raises the challenges of adapting diverse applications onto the hardware platform.
% This would also trigger three issues: 1) Low memory efficiency because of graph traversal overhead and irregular memory accesses; 2) Synchronization stalls in vertex-centric programming model; 3) High input sensitivity (\textit{e.g.}, embedding size, and degree distribution) challenges hardware resources adaption for tasks with different workloads).
% Traditional NNs operate on regular Euclidean data, whereas GNNs operate on non-Euclidean graph data. 
% Even though the computation on each node is still based on regular Euclidean data, node embedding vector, which can leverage data reuse in spatial architectures with horizontal, vertical, or diagonal data flow, 
% In summary, the computations in GNNs are dominated by the NN computing paradigm, while the memory access exhibit both the regular access of Euclidean data and irregular access of non-Euclidean data. The embedding size and the degree distribution of the input graphs affect the computation complexity and the regular/irregular access ratio, thus with different input graphs, GCNs have different favors for graph-style and NN-style computing architectures.  

\textbf{Second, high dimensionality and complex operations inside node feature computation.}
GCNs features high-dimension node/edge embeddding (10x -1000x\cite{KKMMN2016,GraphSage}) with complex NN operation (e.g., Multilayer Perceptron), while the traditional graph computing only works with simple arithmetic operation (e.g., addition) on nodes with scalar value.% Although GNNs shares a similar programming (aggregate and update operations) model as traigraph analytics, 
% Therefore, compared to graph computing, GNNs have complex the computation paradigm and data reuse granularity. 

To this end, we decompose the GCN computing to two parts: intra-node computing on Euclidean data and localized aggregation reduction on non-Euclidean data. We propose a uniform GCN accelerator design, with hierarchical processing element arrays, \Mname, to facilitate an efficient GCN training on both two parts respectively. \Mname integrates the spatial architecture with enhanced memory hierarchy design for both spatial and temporal dataflow optimization. To fully utilize the hardware capability, we propose an hierarchical mapping methodology to improve both the data reuse and task-level parallelism. Specifically,  
justify hierachical. 

%to facilitate an efficient GNN computation on both these two parts. To further improve the 

%The intra-node computing are mainly towards Euclidean data, while localized aggregation reduction are mainly towards non-Euclidean data. We propose a GCN accelerator design, \Mname, to facilitate an efficient GNN computation on both Euclidean and non-Euclidean data. % which supports and optimizes the data reuse of both Euclidean and non-Euclidean data accesses prevalent in GCN. 
%Specifically, \Mname 
%Specifically, our spatial architecture incorporates a novel lightweight graph reordering algorithm and cache hierarchy design to mitigate the irregular memory accesses. And it can also work collaboratively with the existing Euclidean data flow in feature extraction and update. And we decouple the GNN computing to intra-node computing (feature extraction and update) and localized neighboring reduction (aggregation reduction) to handle input diversity,

where we fold the matrix vector multiplications to the multiply-and-Accumulator (MAC) array to handle different feature size and mapping methodology aware of data reuse and task-level parallelism to process graphs with different degree distributions and inherited irregularities.
%  Specifically, we include a lightweight graph reordering algorithm together with the cache hierarchy design in this spatial architectures to mitigate the irregular graph traversal-type memory accesses of non-Euclidean data.  

% To solve the issue of diverse input dataset with different feature size and graph topology, we decouple the GCN computing to intra-node and localized neighboring reduction and propose the mapping methodology aware of data reuse and task-level parallelism to process the input graphs.

Overall, our contributions can be summarized as follows:
\begin{itemize}
        %\item We distinguish the relationships and differences between GNNs, graph computing, and NNs. We identify that graph traversal, synchronization, and diversity of graph data make the GNN accelerations much challenging. 
        %two types of dataflow in GNNs which exhibit both the graph computing and DNN computing models and propose dataflow optimizations for them 
        % (\abanti{abrupt transition from GNN and DNN to GCN and CNN here. Need to change}).  
        % and a lightweight graph re-ordering methodology

      \item We present computing paradigm for GCN workloads, which decouples GCN computing to intra-node computing and localized neighboring reduction.
      \item We design a GCN accelerator, \Mname, that support this paradigm and  the Euclidean and non-Euclidean data reuse in both intra-node computing and localized neighboring reduction.
      %\item We propose a novel lightweight graph reordering algorithm and memory hierarchy design to mitigate the irregular memory accesses in GCN aggregation step.
      \item We incorporates the hierarchical task mapping strategies for intra-node computing and localized reduction, which comprehensively optimize both data reuse and task-level parallelism to well adapt diverse datasets to the hardware platforms. 
      \item Intensive experiments and studies among \Mname, graph, NN accelerator, GPU over a wide range of graph datasets show that \Mname~ outperforms graph, NN accelerator, and GPU with 5.1x, 3.5x, and 7.8x speedup.
  \end{itemize}

% \begin{comment}
%   the computation of which is based on spatial architectures for NN computing accelerations with Euclidean dataflow. Then, we propose the cache hierachy design which augments the accelerators to improve the data reuse of non-Euclidean data. Specifically, for node feature computation exhibits Euclidean dataflow, existing spatial accelerators can be adopted for efficient computation and memory reuse. For the aggregation feature computation exhibit non-Euclidean dataflow, we propose a lightweight graph re-ordering methods accompanied with cache hierarchy design which improve the temporal data reuse. Additionally, the proposed graph re-ordering method also alleviates the workload imbalance issue and reduces the synchronization overhead. 
%  {1. memory access; 2. how to adapt diverse graphs  to static platforms; do not emphasize the workload balance issue.   }
%  {1. spatial architecture with support for hybrid dataflows of non-euclidean data and euclidean data}
 
%  {2. graph reordering to improve data reuse of non-euclidean data}
 
%  {3. mapping algorithm ()
%  to support task-level parallelism and data reuse, different embedding size is folding on MAC array, while different graph size is resolved by the task mapping.}
% \end{comment}
% \begin{comment}
%   \abanti{I think this paragraph needs to be written more carefully. Currently, it is only a list of features with no specific consistency with the challenges mentioned in two prior paragraphs. I think there should be one-to-one correspondence between challenges pointed out in 2 previous paragraphs and the features listed here. Here are some guidelines:
%  \begin{itemize}
%      \item spatial architecture -> is it novel? Which challenge does it solve?
%      \item cache hierarchy -> is it novel? which challenge does it solve?
%      \item graph reordering -> is it novel? which challenge does it solve? 
%      \item how does the accelerator design solve 'Input graph datasets have diverse embedding size and degree distribution?'
%      \item Why is task parallelism and task mapping not mentioned in this paragraph? How does task parallelism or task mapping relate to any of the challenges mentioned in the two prior paragraphs? 
%  \end{itemize}
 
% Here is my suggestion for this paragraph. You can choose whichever is more convenient for you
% Motivated by these challenges, we propose a novel GNN accelerator design, \Mname, which supports and optimizes data reuse for both Euclidean and non-Euclidean data accesses prevalent in GNN. 
% The spatial architecture of our design is in harmony with the Euclidean dataflow in feature extraction and update. 
% To mitigate the irregular graph traversal-type memory accesses in feature reduction (i.e., non-Euclidean dataflow), we include a novel graph reordering algorithm together with a novel cache hierarchy. 
% To solve the synchronization stalls, our design includes............
% To solve the issue of diverse input dataset embeddings, we do ..... blah blah blah
% Finally, to solve the larger data reuse granularity in GNN, we adopt a design philosophy which achieves ..... .blah blah bah
%  }
% \end{comment} 


 
 %with both the Euclidean and non-Euclidean data flow. GNN compute mode Importance questions to answer during characterization  key observations Summary contributions
=============================================


\section{Introduction}
With rich and expressive data representation, graphs demonstrates their applicabilities in various domains, such as E-commerce~\cite{RW-GCN,e-business_1,recommendation_gnn}, computer vision~\cite{vision_gnn1,vision_gnn2},  and molecular structures~\cite{molecular}, and \textit{etc}. To fully exploit the their value, approaches based on traditional graph analytics algorithms (e.g., BFS, SSSP) facilitate in-depth understanding of objects-wise relationships in graphs (\textit{e.g.}, molecule similarity in chemistry~\cite{molecular}, cells structures in bioinformatics~\cite{survey_gnn,GNN_Review}, and parsing an image to semantic graphs~\cite{vision_gnn2,vision_gnn1}).  
%For the ease of , graph embedding provides an effective yet efficient way to solve the graph analytics problem. Specifically, graph embedding converts a graph into a low dimensional space in which the graph information is preserved. By representing a graph as a (or a set of) low dimensional vector(s), graph algorithms
Recently, as a rising star, extending deep learning techniques to graph analytics has gained lots of attention from both research~\cite{GraphSage,1stChebNet,FastGCN,DIFFPOOL} and industry~\cite{AliGraph,googleGraph}, largely because of their striking success on Euclidean data (\textit{e.g.}, images, videos, text, and speech). Moreover, such geometric deep learning techniques based on graph neural networks (GNNs) not only learn the inductive representations for end-to-end tasks such as classification, clustering, and recommendation, but also show much better accuracy (more than 98\%) than traditional methods~\cite{RW-GCN} (\textit{e.g.}, random walks~\cite{deepwalk}, and matrix factorization~\cite{survey_graph_embedding}). 
%Impressed by the capability of capturing the hidden representations of Euclidean data, researchers apply that DNN techniques for graph  applications with non-Euclidean data to learn the inductive representations for end-to-end tasks such as classification, clustering, and recommendation. Such geometric deep learning based on graph neural networks (GNNs) shows its good accuracy compared to the traditional techniques including random works or matrix factorization~\cite{RW-GCN}. 
% \st{Thus GNNs become increasingly important nowadays, with contributions from both academia~\cite{GraphSage,1stChebNet,FastGCN,DIFFPOOL} and industry~\cite{AliGraph,googleGraph}.} 
 \begin{figure}[!htbp]
    \centering
    \includegraphics[scale=0.35]{fig/GNN_comparison.pdf}\vspace{-10pt}
    \caption{Graph, GNN, and NN.}
    \label{fig:gnn_comparison}
\end{figure}

Among diverse GNN algorithms and models~\cite{GraphSage,Adaptive_Sampling}, graph convolutional network (GCN) is the most fundamental and has been widely studied. Different GCNs can be summarized and abstracted into a uniform computing model with two stages: \textit{aggregate} and \textit{update}.
% In this work we focus on the most important one, 
%in also have their potentiality for non-Euclidean data which are represented in the form of graphs. Graph neural networks (GNNs) have been become increasingly important in nowadays.  
%====\Note{GNN algorithm works. the uniform abstraction of computing model.}
%GC
\textbf{\emph{Aggregate}} stage collects the localized node representations from the neighboring nodes through two operations: 1) the \textit{feature extraction} for a single node and 2) the \textit{feature reduction} among neighboring nodes.  
The \textbf{\emph{Update}} stage updates the representation vector based on the aggregation results \todo{and its previous state? unclear}. As shown in Figure~\ref{fig:gnn_comparison}, GCN distinguishes itself by combining graph analytics and neural network computing scheme, where the feature extraction and update involve neural network computation while the feature reduction is essentially a graph traversal. Thus, GCNs computing is confronted with its unique challenges as follows:

\textbf{Hybrid computing paradigm makes the existing NN accelerator and graph accelerator designs pale in effectiveness for handling GCN models}. Specifically, NN accelerators aim to build spatial architectures for powerful computation capabilities while maximizing spatial data reuse~\cite{eyeriss, diannao}. However, GCN localized computing (aggregation reduction) is based on non-Euclidean graph data, which is non-ordered with diverse range of node sizes and topology and introduces the following issues: 
1) Non-Euclidean data introduces irregular memory accesses and synchronization overhead. 2) Non-Euclidean data cannot be easily handled by spatial architectures for spatial data reuse. 
On the other side, graph accelerators prefer resource-intensive on-chip cache to suppress irregular accesses~\cite{graphicionado}. However, GCN has much higher dimensionality and complex operations inside node feature computation. For example, GCNs features high-dimension node/edge embeddding (10x -1000x\cite{KKMMN2016,GraphSage}) with complex NN operation (e.g., Multilayer Perceptron), while the traditional graph computing only works with simple arithmetic operation (e.g., addition) on nodes with scalar value. 
Therefore, an off-the-shelf solution to effectively accelerate GCNs is still missing. Additionally, we may want the GCN accelerator design is in harmony with existing NN accelerator for the practical use.
% GCN computing possesses unique features distinguishable from either, which translates to unique  challenges.
%\abanti{There is some problem with the following two lines: in first line, it is mentioned that GNN = graph + DNN. Immediately, in the next line, we say GNN is different from either. My suggestion is below. You can choose which way you like best}.
%\abanti{Although, GNN may intuitively appear to be a combination of graph analytics and DNN, it possesses unique features distinguishable from either, which translates to unique architecture-level challenges. Thus, existing graph or neural network accelerators are inadequate for GNNs.}
% With different feature dimensions and degree distribution, its behavior shifts towards to graph analytics or CNN computing. 
% CNN 
% Thus, existing graph or neural network accelerators are inadequate for GCNs.
%In summary, GNN incorporates both the computing model of graph and DNN techniques. 
%They exhibit the graph computing model which extracts the localized features among neighboring nodes and the neural network computing model that extracts or embeds the features  hidden states of every node. 
%However, GNNs possess unique features distinguishable from either graph analytics or DNN, which makes existing graph or neural network accelerators inadequate for GNNs.  
%As graph data are often irregular with variable node size and complex topology, some important operations (e.g., convolutions) being easy to compute in the image domain, but difficult to apply to the graph domain.
%\Note{Existing accelerators and conclude they are not good enough for GNNs}
%====\todo{Comparison between graph and GNN, and DNN}.


%\todo{Both the challenges and proposed methods (i.e., our contribution) should be well aligned with our key technical sections: Accelerator, Programming Model and Hardware Primitives, Task Mapping Generation... The challenges focus on why we need these components, while the proposed methods center around the key insights (not technical details) behind how we overcome these challenges. The final contribution bullets would include several key proposed techniques (i.e., the subsection titles) in each key technical sections. }


\textbf{Workload diversity and graph irregularity raises the difficulty to adaptively utilize the hardware capability.} 
%Graph irregularity with variable node volume and feature size raises the challenges of adapting diverse applications onto the hardware platform.
For example, when the input graph has larger feature dimension, the GCN computing shifts to NN computing and demands more MAC arrays for powerful computation capability. However, when the input graph has large scale with high average degrees, the GCN computing demand shifts closer to graph computing that demands large on-chip buffer and date management methodology to eliminate the irregular memory access. Hence, it is important to design the efficient task mapping methodology to bridge the gap between the diverse application demands and uniform hardware platform. 

 

To this end, we first decompose the GCN computing to two parts: 1) node-level computing: intra-node computing (feature extraction and update) on Euclidean data; and 2) graph-level computing: localized neighboring reduction (aggregation reduction) on non-Euclidean data. We propose a uniform GCN accelerator design to facilitate an efficient GCN training on both these two parts respectively. Specifically, \Mname~ propose the hierarchical spatial architecture with cache design to optimize the computing parallelism and data reuse in graph-level computing and node-level computing.
%of both Euclidean and non-Euclidean data. In Geom, MAC arrays are hierarchically organized to processing element (PE) array. PE array provides computing parallelism and temporal dataflow optimization for localized neighboring reduction. While MAC array handles the computation and spatial reuse in the intra-node feature computing. 
%At the top level, the vertexes are allocated into different array for computing parallelism, to provide both the computation parallelism and the dataflow optimization. 
To fully utilize the hardware capability, we propose a hierarchical mapping methodology to improve both the data reuse and task-level parallelism. Specifically, for localized neighboring reduction, Geom maps the node sets with larger potentiality for non-Euclidean data reuse to the same multiply-and-Accumulator (MAC) array based on the locality-sensitive hashing (LSH) clustering techniques. For the intra-node computing, Geom folds the matrix vector multiplications to the multiply-and-Accumulator (MAC) array to handle input graphs with different feature size. 
%and mapping methodology aware of data reuse and task-level parallelism to process graphs with different degree distributions and inherited irregularities.
%justify hierachical. 

%to facilitate an efficient GNN computation on both these two parts. To further improve the 

%The intra-node computing are mainly towards Euclidean data, while localized aggregation reduction are mainly towards non-Euclidean data. We propose a GCN accelerator design, \Mname, to facilitate an efficient GNN computation on both Euclidean and non-Euclidean data. % which supports and optimizes the data reuse of both Euclidean and non-Euclidean data accesses prevalent in GCN. 
%Specifically, \Mname 
%Specifically, our spatial architecture incorporates a novel lightweight graph reordering algorithm and cache hierarchy design to mitigate the irregular memory accesses. And it can also work collaboratively with the existing Euclidean data flow in feature extraction and update. And we decouple the GNN computing to intra-node computing (feature extraction and update) and localized neighboring reduction (aggregation reduction) to handle input diversity,


%  Specifically, we include a lightweight graph reordering algorithm together with the cache hierarchy design in this spatial architectures to mitigate the irregular graph traversal-type memory accesses of non-Euclidean data.  

% To solve the issue of diverse input dataset with different feature size and graph topology, we decouple the GCN computing to intra-node and localized neighboring reduction and propose the mapping methodology aware of data reuse and task-level parallelism to process the input graphs.

Overall, our contributions can be summarized as follows:
\begin{itemize}
        %\item We distinguish the relationships and differences between GNNs, graph computing, and NNs. We identify that graph traversal, synchronization, and diversity of graph data make the GNN accelerations much challenging. 
        %two types of dataflow in GNNs which exhibit both the graph computing and DNN computing models and propose dataflow optimizations for them 
        % (\abanti{abrupt transition from GNN and DNN to GCN and CNN here. Need to change}).  
        % and a lightweight graph re-ordering methodology

      \item We present computing paradigm for GCN workloads, which decouples GCN computing to node-level computing (intra-node feature computing) and graph-level computing (localized neighboring reduction).
      \item We design a GCN training accelerator, \Mname~, based on a hierarchical spatial architecture that supports this paradigm  and  the Euclidean/non-Euclidean data reuse in both node-level computing and graph-level computing.
      %\item We propose a novel lightweight graph reordering algorithm and memory hierarchy design to mitigate the irregular memory accesses in GCN aggregation step.
      \item We incorporates the hierarchical task mapping strategies for intra-node computing and graph-level computing, which comprehensively optimize both data reuse and task-level parallelism to well adapt diverse datasets with different feature size and graph topologies to the hardware platforms. 
      \item Intensive experiments and studies among \Mname, graph, NN accelerator, GPU over a wide range of graph datasets show that \Mname~ outperforms graph, NN accelerator, and GPU with 5.1x, 3.5x, and 7.8x speedup.
  \end{itemize}

% \begin{comment}
%   the computation of which is based on spatial architectures for NN computing accelerations with Euclidean dataflow. Then, we propose the cache hierachy design which augments the accelerators to improve the data reuse of non-Euclidean data. Specifically, for node feature computation exhibits Euclidean dataflow, existing spatial accelerators can be adopted for efficient computation and memory reuse. For the aggregation feature computation exhibit non-Euclidean dataflow, we propose a lightweight graph re-ordering methods accompanied with cache hierarchy design which improve the temporal data reuse. Additionally, the proposed graph re-ordering method also alleviates the workload imbalance issue and reduces the synchronization overhead. 
%  {1. memory access; 2. how to adapt diverse graphs  to static platforms; do not emphasize the workload balance issue.   }
%  {1. spatial architecture with support for hybrid dataflows of non-euclidean data and euclidean data}
 
%  {2. graph reordering to improve data reuse of non-euclidean data}
 
%  {3. mapping algorithm ()
%  to support task-level parallelism and data reuse, different embedding size is folding on MAC array, while different graph size is resolved by the task mapping.}
% \end{comment}
% \begin{comment}
%   \abanti{I think this paragraph needs to be written more carefully. Currently, it is only a list of features with no specific consistency with the challenges mentioned in two prior paragraphs. I think there should be one-to-one correspondence between challenges pointed out in 2 previous paragraphs and the features listed here. Here are some guidelines:
%  \begin{itemize}
%      \item spatial architecture -> is it novel? Which challenge does it solve?
%      \item cache hierarchy -> is it novel? which challenge does it solve?
%      \item graph reordering -> is it novel? which challenge does it solve? 
%      \item how does the accelerator design solve 'Input graph datasets have diverse embedding size and degree distribution?'
%      \item Why is task parallelism and task mapping not mentioned in this paragraph? How does task parallelism or task mapping relate to any of the challenges mentioned in the two prior paragraphs? 
%  \end{itemize}
 
% Here is my suggestion for this paragraph. You can choose whichever is more convenient for you
% Motivated by these challenges, we propose a novel GNN accelerator design, \Mname, which supports and optimizes data reuse for both Euclidean and non-Euclidean data accesses prevalent in GNN. 
% The spatial architecture of our design is in harmony with the Euclidean dataflow in feature extraction and update. 
% To mitigate the irregular graph traversal-type memory accesses in feature reduction (i.e., non-Euclidean dataflow), we include a novel graph reordering algorithm together with a novel cache hierarchy. 
% To solve the synchronization stalls, our design includes............
% To solve the issue of diverse input dataset embeddings, we do ..... blah blah blah
% Finally, to solve the larger data reuse granularity in GNN, we adopt a design philosophy which achieves ..... .blah blah bah
%  }
% \end{comment} 


 
 %with both the Euclidean and non-Euclidean data flow. GNN compute mode Importance questions to answer during characterization  key observations Summary contributions

